Deep Stereo using Adaptive Thin Volume Representation with Uncertainty Awareness

We present Uncertainty-aware Cascaded Stereo Network (UCS-Net) for 3D reconstruction from multiple RGB images. Multi-view stereo (MVS) aims to reconstruct fine-grained scene geometry from multi-view images. Previous learning-based MVS methods estimate per-view depth using plane sweep volumes with a fixed depth hypothesis at each plane; this generally requires densely sampled planes for desired accuracy, and it is very hard to achieve high-resolution depth. In contrast, we propose adaptive thin volumes (ATVs); in an ATV, the depth hypothesis of each plane is spatially varying, which adapts to the uncertainties of previous per-pixel depth predictions. Our UCS-Net has three stages: the first stage processes a small standard plane sweep volume to predict low-resolution depth; two ATVs are then used in the following stages to refine the depth with higher resolution and higher accuracy. Our ATV consists of only a small number of planes; yet, it efficiently partitions local depth ranges within learned small intervals. In particular, we propose to use variance-based uncertainty estimates to adaptively construct ATVs; this differentiable process introduces reasonable and fine-grained spatial partitioning. Our multi-stage framework progressively subdivides the vast scene space with increasing depth resolution and precision, which enables scene reconstruction with high completeness and accuracy in a coarse-to-fine fashion. We demonstrate that our method achieves superior performance compared with state-of-the-art benchmarks on various challenging datasets.

==> experiments.tex <==
We evaluate our UCS-Net with various experiments.
We compare our method with state-of-the-art benchmarks, and observe qualitatively and quantitatively best performance.
We also evaluate our system with different configurations, in terms of the number of stages and the number of sweeping planes per stage.

\subsection{Implementation Details}
\label{sec: impl}
We now introduce the details of our implementation of the UCS-Net.

\noindent\textbf{Parameters} We choose DPSNet \cite{im2018dpsnet} (with 64 depth levels) as our unit network in Figure \ref{fig:ucnet} since it achieves the best state-of-the-art performance to our knowledge. For all our experiments, we use $\lambda=1.5$ (in Eqn.~\eqref{eqn:interval}), $d_\text{min}=0.5$ (in Eqn.~\eqref{eqn:depthDisp}), $L_\text{max}=64$ (in Eqn.~\eqref{eqn:depthDisp}) and $\beta=0.7$ (in Eqn.~\eqref{eqn:loss}). 

\noindent\textbf{Dataset} We split the SUN3D \cite{xiao2013sun3d}, RGBD \cite{sturm2012benchmark} and Scenes11 \cite{ummenhofer2017demon, chang2015shapenet} datasets into training sets and testing sets in the same way as \cite{im2018dpsnet}.
We train our networks on the three training sets (SUN3D, RGBD, Scenes11), and test them on the three testing sets (SUN3D, RGBD, Scenes11). We also include one additional test dataset (MVS \cite{schonberger2016structure, schonberger2016pixelwise}) for generalizability evaluation with no training. 

\noindent\textbf{Metric} Following the convention of DPSNet, we compute several common quantitative depth measurements: absolute relative error (Abs Rel), absolute relative inverse error (Abs R-Inv), absolute difference error (Abs diff), square relative error (Sq Rel), root mean square error (RMSE) and its log scale (RMSE log), and inlier
ratios ($\alpha$, $\alpha^{2}$, $\alpha^{3}$).

\noindent\textbf{Training} We train our network with ADAM optimizer with a batch size of 8; the initial learning rate is set to 0.0002. 
We use Nvidia 1080Ti GPUs to train all networks.
To facilitate the training convergence, we use the weights of a pre-trained DPSNet (trained with 64 planes) as the common initial weights to train all cascade stages in different configurations. 
Our first stage converges after 5 epochs; our second and third stages generally converge after 2 epochs.




\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{images/ICCV_compare.pdf}
	\caption{Qualitative comparisons. We show comparisons between our 32-16 UCS-Net and DPSNet. We show a few zoomed-in insets from the original images to illustrate the visual differences.}
	\label{fig:compare}
	\vspace{-3mm}
\end{figure*}

\subsection{Comparing with State-of-the-art Baselines}
\label{sec: comp}
We train our UCS-Net with two 2-stage configurations, 32-32 and 32-16, where X-Y describes the number of sweeping planes in a volume (that is either a standard plane sweep volume or an adaptive thin volume, e.g. $32-16$ corresponds to a 2-stage UCS-Net trained with $32$ planes in the first stage and $16$ planes in the second stage).
We compare our UCS-Nets (32-32, 32-16) with various state-of-the-art MVS approaches including the traditional geometry-based multiview stereo (COLMAP \cite{schonberger2016structure}), unstructured binocular stereo (DeMoN \cite{ummenhofer2017demon}), classification-based deep stereo (DeepMVS \cite{huang2018deepmvs}), and regression-based deep stereo (DPSNet \cite{im2018dpsnet}).
Since our multi-stage UCS-Net has larger network capacity than DPSNet, we train and compare an extra DPSNet with double capacity (that we refer to as DPSNet-DC), for which we copy each convolutional layer of the DPSNet as an extra layer appended to the original one.
This is a simple strategy that trivially increases the network capacity; we compare our UCS-Nets with this double-capacity DPSNet to verify that our significant performance gain does not come from our increased network capacity of multiple stages. 
We train the DPSNet-DC with the same setting as the DPSNet as reported in \cite{im2018dpsnet}; we take the network with 12 epochs, which already converges.


We compare the performance of all methods on the test data of MVS, SUN3D, RGBD and Scenes11 datasets.
Since we apply the same testing set as \cite{im2018dpsnet}, we use the reported performance of COLMAP \cite{schonberger2016structure}, DeMoN \cite{ummenhofer2017demon}, DeepMVS \cite{huang2018deepmvs} from Tab.~1 in \cite{im2018dpsnet}.
For DPSNet, we use the authors' newly updated trained model and reported performance metrics on their website (\url{https://github.com/sunghoonim/DPSNet}), which are overall better than the original ones reported in Tab.~1 of \cite{im2018dpsnet}.
For our networks and the DPSNet-DC, we evaluate them on the same testing datasets with the same setting as \cite{im2018dpsnet}.
We calculate the averaged values (weighted by the sizes of datasets) of all metrics across all datasets, and
the results are reported in Tab.~\ref{tab: alldata}.
We also visualize the comparisons between our UCS-Nets, DPSNet and DPSNet-DC with four most common metrics with bar plots, as shown in Fig.~\ref{fig:bar_overall}. 
For detailed comparisons of individual datasets, please refer to the supplemental material.

The results reveal that our UCS-Nets both consistently perform better than the other methods for nearly all of the 8 computed metrics, with the gain up to $12\%$. 
This illustrates the high performance of our UCS-Nets, which leverage the novel adaptive thin volumes (ATVs) to effectively sub-partition the local space and push the limit of depth estimation.
We also observe that our 32-32 configuration achieves better results than our 32-16, which is expected since the 32-32 UCS-Net partitions the local space with a higher disparity resolution.
For more ablation studies, please refer to Sec.~\ref{sec: abl}.
Note that, our 32-16 UCS-Net merely utilizes 48 sweeping planes in total; while it performs worse than our 32-32 UCS-Net, it is still consistently better than DPSNet and DPSNet-DC with 64 (that is $33\%$ more than our 48) sweeping planes.
To highlight our improvement over DPSNet,  Figure.~\ref{fig:compare} shows qualitative comparisons between our 32-16 UCS-Net and DPSNet; our method achieves better depth reconstruction with more accurate details.
This favorable comparison clearly justifies the effectiveness and high accuracy of our coarse-to-fine approach, and demonstrates that our UCS-Net is able to achieve better performance with less memory and computation.

Moreover, the results of DPSNet vs DPSNet-DC show that depth reconstruction cannot be improved with a deeper network that is simply achieved by stacking repeated layers; the over-sized network has serious issues of overfitting, and, in fact, even has a few metrics that are lower than the original DPSNet's.
In contrast, our UCS-Nets improve the performance of DPSNet by a large margin, with the same network capacity as DPSNet-DC; this demonstrates that our UCS-Nets are able to utilize the same network capacity in a more reasonable way, which leverage better spatial representations.
This experiment demonstrates that our high performance is \textit{not} because of making the network deeper, \textit{but} because of our novel cascaded network with the novel thin volume representation, which, as a whole, progressively attains highly accurate depth reconstruction via a coarse-to-fine process. 


\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{images/ICCV_ablation.pdf}
	\caption{Multi-stage details. We show two results from our 32-16. From left to right, we show the RGB images of the reference views, ground truth depth maps, our final predicted depth maps, the disparity distributions of the first and second stages for two pixels (green). The ground truth and predicted disparity surrounded by the confidence intervals are also shown in the distributions, similar to Fig.~\ref{fig:method}.}
	\label{fig:ablation}
\end{figure*}

\begin{table*}[th!]
	\footnotesize
	\centering
	\begin{tabular}[width=\linewidth]{p{1.8cm}p{2.2cm}p{0.9cm}p{1cm}p{0.9cm}p{0.9cm}p{1.3cm}p{0.8cm}p{0.8cm}p{0.8cm}}
		\Xhline{2pt}
		Method & Config & Abs Rel & Abs Diff & Sq Rel & RMSE & RMSE log & $\alpha$ & $\alpha^{2}$ & $\alpha^{3}$\\ 
		\Xhline{2pt}
		DPSNet & 64 & 0.1005 & 0.2880 & 0.1413 & 0.5095 & 0.1707 & 0.8709 & 0.9430 & 0.9680\\
		
		UnitNet & 32 & 0.1045&	0.2899&	0.1469&	0.5162&	0.1696&	0.8825&	0.9506&	0.9725\\
		
		\Xhline{2pt}
		
		UCS-Net & 32-32 & 0.0913 &0.2658 &0.1197 &0.4790 &0.1606 &0.8922 &0.9545 &0.9753\\
		
		UCS-Net & 32-16 & 0.0919 &0.2738 &0.1218 & 0.4840& 0.1633& 0.8872& 0.9501& 0.9717\\
		
		%UCS-Net & 32-16 & ATV+Disp & 0.0923& 0.2683& 0.1221& 0.4859& 0.1633& 0.8874& 0.9527& 0.9733\\
		
		\Xhline{2pt}
		
		UCS-Net & 32-16-16 & 0.0916&     0.2702&     0.1212&     0.4811&     0.1619&     0.8889&     0.9512&     0.9723\\
		
		%UCS-Net & 32-16-16 & ATV+Disp & & & & & & & & \\
		
		\Xhline{2pt}
		
	\end{tabular}
	\vspace{+1mm}
	\caption{Comparisons using UCS-Net with different configurations.}
	\label{tab: ablation}
	\vspace{-3mm}
\end{table*}

\subsection{Comparing UCS-Net Configurations}
\label{sec: abl}
We evaluate our UCS-Net with various configurations to verify the effectiveness of our framework. 
In particular, we train the UCS-Net with one (that is the original DPSNet setting), two, and three stages, also with different number of sweeping planes.

We show the relative memory usage and disparity resolution of these configurations in Tab.~\ref{tab: config}.
Since we utilize smaller numbers of sweeping planes in our volumes, our UCS-Net halves the maximum memory usage of DPSNet.
Nevertheless, our ATV representation enables spatial partitioning at a resolution that is much higher than DPSNet, which further enables highly accurate depth reconstruction.

We test all networks on our test dataset and show the quantitative results in Tab.~\ref{tab: ablation}.
We compare different numbers of sweeping planes with the same number of stages, i.e. UCS-Net-32-16 vs UCS-Net-32-32; our UCS-Net performs better when it uses more planes to partition the space at a stage (which has already been demonstrated in Sec.~\ref{sec: comp}).
Besides, our framework consistently performs better when it has more stages, as shown in the results of  32 (UnitNet) vs 32-16, 32 (UnitNet) vs 32-32, and 32-16 vs 32-16-16.
This verifies that our UCS-Net with ATVs effectively utilizes the uncertainty of per-stage prediction and enables accurate depth estimation.
Figure.~\ref{fig:ablation} shows the reconstruction details of single points; the reliable uncertainty inference enables the construction of a thin volume around the ground truth depth in a narrow disparity range, which further enables more accurate estimation.

We demonstrate that increasing the number of stages is a very efficient way to improve the performance, since an extra ATV can sub-partition the local space at a finer scale; this allows that our 32-32 and 32-16 UCS-Net achieves much better results than the DPSNet with 64 planes.
As discussed, our multi-stage UCS-Nets use the same or even a smaller number of planes, but performs much better than the original DPSNet.
Note that, the prediction of 32-16 has a much larger uncertainty than 32-32, corresponding to a much lower disparity resolution as shown Tab.~\ref{tab: config}. 
This large uncertainty cannot be rapidly reduced by a third 16-plane stage; as a result, our 32-16-16 UCS-Net performs slightly worse than the 32-32 UCS-Net.
Potentially, given a fixed number of total planes, there is a trade-off between the number of stages and the number of per-stage sweeping planes; we leave the development of optimal configurations to future work.







\begin{table}[th!]
	\footnotesize
	\centering
	\begin{tabular}[width=\linewidth]{p{2cm}p{2cm}p{1cm}p{1cm}}
		\Xhline{2pt}
		Method & Config & Res & Memory\\ 
		\Xhline{2pt}
		DPSNet (Base) & 64 & 1x & 1x\\
		
		DPSNet-DC & 64 & 1x & $\sim$2x\\
		
		UnitNet & 32 & 2x & \textbf{$\sim$0.5x}\\
		
		UCS-Net & 32-32 & \textbf{$\sim$0.0861x} & \textbf{$\sim$0.5x}\\
		
		UCS-Net & 32-16 & $\sim$0.1723x & \textbf{$\sim$0.5x}\\
		
		UCS-Net & 32-16-16 & $\sim$0.1315x & \textbf{$\sim$0.5x}\\
		
		\Xhline{2pt}
	\end{tabular}
	\vspace{+1mm}
	\caption{The disparity resolution and maximum memory usage of different configurations.}
	\vspace{-0.12in}
	\label{tab: config}
\end{table}


\subsection{Limitations and Future Work}
We briefly discuss limitations. 
Our UnitNet is currently based on a previous learning-based MVS system for depth regression; in general, we have similar limitations to other learning-based methods, which are limited to the quality of training data.
We observe that methods along this line of work still have difficulty in recovering challenging scene boundary regions that have two peaks in disparity distributions.
Increasing the number of input views generally improves the quality.
Besides, since we are using a coarse-to-fine framework, when an incorrect prediction is far away from the ground truth and out of the predicted uncertainty boundary, it cannot be corrected in later stages. 

We apply traditional probability analysis in a learning-based coarse-to-fine framework; we believe this general idea can potentially inspire future work on various learning-based methods.
In particular, we believe our novel uncertainty-aware spatial partitioning strategy is insightful for 3D deep learning;
it's interesting to explore if our ATV representation can be applied to resolve other problems, like point-cloud-based 3D reconstruction, novel view synthesis and even single image 3D reconstruction.

